Graphulo Implementation of Server-Side Sparse Matrix Multiply in the Accumulo Database

The Apache Accumulo database excels at distributed storage and indexing and is ideally suited for storing graph data. Many big data analytics compute on graph data and persist their results back to the database. These graph calculations are often best performed inside the database server. The GraphBLAS standard provides a compact and efficient basis for a wide range of graph applications through a small number of sparse matrix operations. In this article, we implement GraphBLAS sparse matrix multiplication server-side by leveraging Accumulo's native, high-performance iterators. We compare the mathematics and performance of inner and outer product implementations, and show how an outer product implementation achieves optimal performance near Accumulo's peak write rate. We offer our work as a core component to the Graphulo library that will deliver matrix math primitives for graph analytics within Accumulo.

==> Makefile <==
# input file name.  This defines the name of the file you want to latex
# the make file will automatically look for INPUT.tex as the latex file
# and will look for a INPUT.bib file for the bibliography
INPUT=Graphulo_2015_HPEC_MatrixMultiply
BIBFILE=10_bibliography

#commands 
TEX=latex
PDFTEX=pdflatex
LYX=lyx
BIBTEX=bibtex
DVIPS=dvips -t letter
PS2PDF=ps2pdf14 -dPDFSETTINGS=/prepress

#extensions
DVIEXT=.dvi
PSEXT=.ps
TEXEXT=.tex
BIBEXT=.bib
LYXEXT=.lyx
PDFEXT=.pdf

default: pdf

dvi: latex bibtex latex2

latex: 
	$(TEX) $(INPUT)$(TEXEXT)

latex2:
	$(TEX) $(INPUT)$(TEXEXT)
	$(TEX) $(INPUT)$(TEXEXT)

pdflatex: 
	$(PDFTEX) $(INPUT)$(TEXEXT)

pdflatex2:
	$(PDFTEX) $(INPUT)$(TEXEXT)
	$(PDFTEX) $(INPUT)$(TEXEXT)

bibtex: $(BIBFILE)$(BIBEXT) 
	$(BIBTEX) $(INPUT)

ps: dvi
	$(DVIPS) -o $(INPUT)$(PSEXT) $(INPUT)$(DVIEXT)

pspdf: ps
	$(PS2PDF) $(INPUT)$(PSEXT)

pdf: pdflatex bibtex pdflatex2

gentex:
	$(LYX) --export latex $(INPUT)-lyx$(LYXEXT)

viewdvi:
	kdvi $(INPUT)$(DVIEXT)

view: kpdf

kpdf:
	okular $(INPUT)$(PDFEXT)

clean:
	rm -f $(INPUT)$(PSEXT)
	rm -f $(INPUT)$(DVIEXT) 
	rm -f *.aux *.bbl *.blg *.log *.toc

cleaner: clean
	rm -f *~
	rm -f $(INPUT)$(PDFEXT)

arxiv: # flatten directories
	cp $(INPUT).bbl $(BIBFILE).bbl
	tar --transform 's/.*\///g' -czf $(INPUT)_arxiv.tar.gz 00_abstract.tex 01_introduction.tex 02_design.tex 03_performance.tex 04_conclusions.tex 10_bibliography.bib img/TableMultRate.eps img/TableMultIteratorStack.pdf img/InnerOuterSpectrum.pdf Graphulo_2015_HPEC_MatrixMultiply.tex Makefile $(BIBFILE).bbl

